HoliSDiP: Image Super-Resolution via Holistic Semantics and Diffusion Prior

Text-to-image diffusion models have emerged as powerful priors for real-world image super-resolution (Real-ISR). However, existing methods may produce unintended results due to noisy text prompts and their lack of spatial information. In this paper, we present HoliSDiP, a framework that leverages semantic segmentation to provide both precise textual and spatial guidance for diffusion-based Real-ISR. Our method employs semantic labels as concise text prompts while introducing dense semantic guidance through segmentation masks and our proposed Segmentation-CLIP Map. Extensive experiments demonstrate that HoliSDiP achieves significant improvement in image quality across various Real-ISR scenarios through reduced prompt noise and enhanced spatial control.

==> Figures/ablation_seg-quality.tex <==
\begin{figure}[t]
    \centering

    % First row - Integrated Guidance section
    \vspace{1mm}
    \begin{subfigure}[b]{0.192\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/a-1.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.192\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/a-2.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.192\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/a-3.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.192\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/a-4.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.192\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/a-5.pdf}
    \end{subfigure}

    \vspace{-0.3mm}

    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/b-1.pdf}
        \caption*{\centering \scriptsize LR Image}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/b-2.pdf}
        \caption*{\centering \scriptsize Mask2Former~\cite{mask2former} (Swin-T)}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/b-3.pdf}
        \caption*{\centering \scriptsize Mask2Former~\cite{mask2former} (Swin-B)}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/ablation-seg-quality/b-4.pdf}
        \caption*{\centering \scriptsize Mask2Former~\cite{mask2former} (Swin-L)}}
    \end{subfigure}
    \caption{Semantic segmentation masks generated by Mask2Former~\cite{mask2former} with different backbones.}
    \label{fig:ablation_seg-quality}
\end{figure}


==> Figures/teaser.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_vertical_2row.pdf}
%   \caption{
%     (a) Our proposed framework integrates vision and language guidance, effectively reducing hallucinations and enhancing semantic consistency of objects. (b) Our approach provides concise object descriptions by employing semantic segmentation labels as text prompts, which greatly reduces artifacts and eliminates the need for a separate prompt generation module.
%   }
%   \label{fig:teaser}
% \end{figure}
\begin{figure}[t]
    \centering
    
    \centerline{\scriptsize (a) The influence of unifying vision and language guidance}
    
    % First row - Integrated Guidance section
    \vspace{1mm}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_a-1-new.pdf}
        \caption*{\centering \scriptsize LR Image}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_a-2-new.pdf}
        \caption*{\centering \scriptsize w/o Unified Guidance}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_a-3-new.pdf}
        \caption*{\centering \scriptsize \textcolor{red}{w/ Unified Guidance (Ours)}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_a-4-new.pdf}
        \caption*{\centering \scriptsize Ground Truth}}
    \end{subfigure}

    % Text below the first row 
    \vspace{2mm}

    \centerline{\scriptsize (b) The effect of employing our Semantic Label-Based Prompting (SLBP)}

    % Second row - Semantic Labels section
    \vspace{1mm}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_b-1-new.pdf}
        \caption*{\centering \scriptsize LR Image}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_b-2-new.pdf}
        \caption*{\centering \scriptsize w/ Image Tags~\cite{seesr}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_b-3-new.pdf}
        \caption*{\centering \scriptsize \textcolor{red}{w/ SLBP (Ours)}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
        \vtop{\centering
        \includegraphics[width=\linewidth]{Figures/Images/teaser/teaser_b-4-new.pdf}
        \caption*{\centering \scriptsize Ground Truth}}
    \end{subfigure}

    \caption{(a) Our proposed framework effectively integrates vision and language guidance, mitigating hallucinations and enhancing semantic consistency of objects. (b) The proposed SLBP scheme provides concise object descriptions, greatly reducing artifacts.}
    % and eliminates the need for a separate prompt generation module~\cite{ram, llava}.}
    \label{fig:teaser}
\end{figure}


